Fidelity-Aware Scheduling of Quantum Circuits on Multi-QPU Systems

High Performance Computing-Quantum Computing (HPCQC) platforms expose multiple Quantum Processing Units (QPUs) that may differ in size, topology, native gates, and noise characteristics. For current noisy devices, errors compound along the compiled circuits quickly, and minimizing them, that is, maximizing the circuits' execution fidelity, is essential for reliable results. Fidelity depends on the compilation to a specific target device: the same high-level circuit may produce different executables and, therefore, different expected fidelities across QPUs. We present a low-overhead fidelity-aware scheduling framework for multi-QPU systems based on a Graph Neural Network (GNN) that estimates, before compilation, the expected fidelity of each circuit on each available QPU. Then, a tunable scheduler uses these estimates to control the trade-off between execution fidelity and parallelism. Results show that this framework allows for approximating an exhaustive fidelity-based assignment, saving computational resources compared to a brute-force approach that compiles each circuit on every device.

==> imgs/circuitkz/gnn_architecture.tex <==
% GNN architecture diagram for the HPC-QC device predictor.
%
% Model parameters (optuna_results/best_params.json):
%   hidden_dim          = 61
%   num_conv_wo_resnet  = 3
%   num_resnet_layers   = 9
%   dropout             = 0.0
%   bidirectional       = False
%   mlp                 = [256, 128, 64]
%   readout             = meanmaxsum  →  61 × 3 = 183
%   output_dim          = 3
%
% Input feature dimension: len(get_openqasm3_gates()) + 1 + 6 + 3 + 1 + 1 + 1 = 39


\begin{tikzpicture}[node distance=4.5mm]

% ── 1. Non-residual encoder ────────────────────────────────────────────────────

\node[conv] (c1)
  {SAGEConv \;$39\!\to\!61$\quad GraphNorm\quad LeakyReLU};

\node[conv, below=of c1] (c2)
  {SAGEConv \;$61\!\to\!61$\quad GraphNorm\quad LeakyReLU};

\node[conv, below=of c2] (c3)
  {SAGEConv \;$61\!\to\!61$\quad GraphNorm\quad LeakyReLU};

% right-side brace + label
\draw[decorate,
      decoration={calligraphic brace, amplitude=5pt, raise=5pt},
      line width=0.6pt]
  (c1.north east) -- (c3.south east)
  node[midway, right=11pt, seclabel, font=\Large\bfseries, align=left]
    {non-residual\\$\times 3$};

% ── 2. Residual encoder ────────────────────────────────────────────────────────

\node[resconv, below=10mm of c3] (res)
  {SAGEConv \;$61\!\to\!61$\quad GraphNorm\quad LeakyReLU\quad
   $\oplus\;\mathbf{x}$\;(\textit{skip})};

\node[right=0.55cm of res, seclabel, font=\Large\bfseries, align=left] (reslabel)
  {residual\\$\times 9$};

% residual bypass arrow (left side)
%\draw[resarr]
%  ([xshift=-7mm] res.north west) coordinate (rtop)
%  -- ([xshift=-7mm] res.south west) coordinate (rbot);
%\node[left=0pt of rtop, dimtag, font=\Large\itshape, inner sep=1pt] {$\mathbf{x}$};
%\node[left=0pt of rbot, dimtag, font=\Large\itshape, inner sep=1pt] {$+$};

% ── 3. Readout ─────────────────────────────────────────────────────────────────

\node[pool, below=10mm of res] (pool)
  {{\Large MeanMaxSum Pooling \quad
   $\mathbf{h}_v\!\in\!\mathbb{R}^{61}
    \;\xrightarrow{\;\text{mean}\oplus\text{max}\oplus\text{sum}\;}
    \;\mathbf{g}\!\in\!\mathbb{R}^{183}$}};

% ── 4. MLP head ────────────────────────────────────────────────────────────────

\node[mlp, below=10mm of pool] (fc1)
  {Linear \;$183\!\to\!256$\quad LeakyReLU};

\node[mlp, below=of fc1] (fc2)
  {Linear \;$256\!\to\!128$\quad LeakyReLU};

\node[mlp, below=of fc2] (fc3)
  {Linear \;$128\!\to\!64$\quad LeakyReLU};

% ── 5. Output head ─────────────────────────────────────────────────────────────

\node[outbox, below=10mm of fc3] (outlin)
  {Linear \;$64\!\to\!3$};

% three output nodes
\node[smallout, below left =9mm and -3.3cm of outlin] (o1) {EQE1\_Top};
\node[smallout, below       =9mm             of outlin] (o2) {EQE1\_Bottom};
\node[smallout, below right =9mm and -3.3cm  of outlin] (o3) {QExa20};

% ── Arrows ─────────────────────────────────────────────────────────────────────

% input arrow
\draw[arr] ([yshift=10mm]c1.north) -- (c1.north)
  node[above, font=\Large, align=center]
    at ([yshift=10mm]c1.north)
    {Input graph \quad node features $\mathbf{x}_v\in\mathbb{R}^{39}$};

% encoder chain
\foreach \a/\b in {c1/c2, c2/c3}
  \draw[arr] (\a.south) -- (\b.north);

\draw[arr] (c3.south)    -- (res.north);
\draw[arr] (res.south)   -- (pool.north);
\draw[arr] (pool.south)  -- (fc1.north);
\foreach \a/\b in {fc1/fc2, fc2/fc3}
  \draw[arr] (\a.south) -- (\b.north);
\draw[arr] (fc3.south)   -- (outlin.north);

% fan-out to output nodes
\draw[arr] (outlin.south) -- (o1.north);
\draw[arr] (outlin.south) -- (o2.north);
\draw[arr] (outlin.south) -- (o3.north);

% ── Background section boxes ───────────────────────────────────────────────────

\begin{scope}[on background layer]
  \node[fill=blue!5, rounded corners=5pt,
        fit=(c1)(c3), inner sep=7pt,
        label={[seclabel, font=\Large\bfseries, text=blue!50, anchor=west, xshift=7pt]above:GNN Encoder — non-residual}] {};

  \node[fill=orange!5, rounded corners=5pt,
        fit=(res), inner sep=7pt,
        label={[seclabel, font=\Large\bfseries, text=orange!60, anchor=west, xshift=7pt]above:GNN Encoder — residual}] {};

  \node[fill=violet!5, rounded corners=5pt,
        fit=(fc1)(fc3), inner sep=7pt,
        label={[seclabel, font=\Large\bfseries, text=violet!60, anchor=west, xshift=7pt]above:MLP Head}] {};
\end{scope}

\end{tikzpicture}
